On the asymptotic magnitude of subsets of Euclidean space

Magnitude is a canonical invariant of finite metric spaces which has its origins in category theory; it is analogous to cardinality of finite sets. Here, by approximating certain compact subsets of Euclidean space with finite subsets, the magnitudes of line segments, circles and Cantor sets are defined and calculated. It is observed that asymptotically these satisfy the inclusion-exclusion principle, relating them to intrinsic volumes of polyconvex sets.

==> CantorMagGraph.table.tex <==
0	1
0.2179715416	1.108968519
0.4076274145	1.203701016
0.6209152791	1.310060253
0.835616954	1.416843009
1.049298189	1.522745311
1.247408048	1.62052035
1.452539331	1.721271103
1.664686398	1.824869012
1.876153106	1.92745665
2.093672608	2.032203503
2.285263904	2.12375916
2.500950325	2.225985055
2.717522375	2.327680685
2.926229675	2.424739652
3.115755897	2.512046212
3.341120908	2.614799928
3.532034633	2.70092216
3.754112681	2.800017473
3.950689383	2.88674799
4.166365181	2.98083209
4.371739543	3.069375632
4.586026145	3.160673939
4.782808139	3.24354039
4.995064103	3.331885958
5.215538397	3.42252507
5.407461918	3.500504382
5.614744578	3.583775345
5.828887849	3.66878628
6.038385262	3.75097418
6.24108478	3.829594359
6.466148036	3.915875968
6.668377382	3.99251814
6.884300374	4.07345
7.079958697	4.146005507
7.293864924	4.224502899
7.495134013	4.297598776
7.705518205	4.37323718
7.911207207	4.44645193
8.12654453	4.522346368
8.333939965	4.594735255
8.546031753	4.66806967
8.756367313	4.740126478
8.949643849	4.805769284
9.171160569	4.88035361
9.369287765	4.946493243
9.58053268	5.016438582
9.782721017	5.082848147
10	5.153647204


==> CantorMagValuationGraph.table.tex <==
0	0
0.1056831717	0.2920499827
0.1976375343	0.4333580148
0.3010498323	0.5653353685
0.4051476141	0.681659149
0.5087506373	0.786857659
0.604803902	0.877659613
0.7042614939	0.9663122365
0.8071206777	1.05323147
0.9096499908	1.135796872
1.015113992	1.217115382
1.108006741	1.286132232
1.212581976	1.361296447
1.317586606	1.43440655
1.418778024	1.502884412
1.510669526	1.56355936
1.61993741	1.634011255
1.71250164	1.692368484
1.820175845	1.758841044
1.915485761	1.816499934
2.020055845	1.878568156
2.119631294	1.936580638
2.223527828	1.996041815
2.31893728	2.04973673
2.421849262	2.106730595
2.52874589	2.164970324
2.621799718	2.214912368
2.722300402	2.268101084
2.826127442	2.322272816
2.927701945	2.374543288
3.0259805	2.424467958
3.135102078	2.479189191
3.23315267	2.52775066
3.337842606	2.578995684
3.432707247	2.624916201
3.536419357	2.674584144
3.63400437	2.720828957
3.736008827	2.768682924
3.835736828	2.815008925
3.940142803	2.863040222
4.040698165	2.908865246
4.143530547	2.955303326
4.245511425	3.000948102
4.33922126	3.042544228
4.446623307	3.089823304
4.542684977	3.13176427
4.645106754	3.176133415
4.743137463	3.218273114
4.851987967	3.264699789
4.946244506	3.30460089
5.05322652	3.349559749
5.150729012	3.390237701
5.257381415	3.434416766
5.349404401	3.472276578
5.454207842	3.515108858
5.555442791	3.556200394
5.656611607	3.596994168
5.75740824	3.637374378
5.854242249	3.675924601
5.958922377	3.717336636
6.05869013	3.756557311
6.163690991	3.797579152
6.258742056	3.834491742
6.363791276	3.875046388
6.464410124	3.913658236
6.564784062	3.951953829
6.66962503	3.99172116
6.766187388	4.02814198
6.865080452	4.065240532
6.974270145	4.105969396
7.073132468	4.142639562
7.174237711	4.17994243
7.27705914	4.217675534
7.371572041	4.252182234
7.472319733	4.288781434
7.572300527	4.324917716
7.679248898	4.363372658
7.773626203	4.397139041
7.882518021	4.435905704
7.980784492	4.470715424
8.078014028	4.50499797
8.182567015	4.541688316
8.287542941	4.578348388
8.383055489	4.61155072
8.484485573	4.646653305
8.583471421	4.680756824
8.690773125	4.717557406
8.783618932	4.749261433
8.890255717	4.785518548
8.990499901	4.819452436
9.089775835	4.852917952
9.189130745	4.886272254
9.290466463	4.92015178
9.397880626	4.955911956
9.496368896	4.988565704
9.593589465	5.02067466
9.697516653	5.054863975
9.8012176	5.08884239
9.894295359	5.119225745
10	5.153601805


==> CircleDistanceGraphkappa-10.dat.tex <==
0	0
0.01089857708	0.0108752777
0.02179715417	0.02161365363
0.03127994781	0.03074914973
0.04076274146	0.03962039555
0.05142713469	0.04921882393
0.06209152792	0.05837151925
0.07282661167	0.06710957641
0.08356169542	0.07536409166
0.104929819	0.09039158547
0.1247408048	0.1027661188
0.1452539331	0.1141651251
0.1664686398	0.1246184671
0.1876153106	0.1338526447
0.2093672608	0.1422667398
0.2285263904	0.1488695888
0.2500950325	0.1554928475
0.2717522375	0.1613641926
0.2926229675	0.1663512194
0.3115755898	0.1703547333
0.3341120908	0.1745117255
0.3532034633	0.1775523296
0.3754112681	0.1805663058
0.3950689383	0.1827872043
0.4166365181	0.184761082
0.4371739544	0.186205439
0.4586026146	0.1872717772
0.478280814	0.1878618474
0.4995064104	0.188085296
0.5215538398	0.1878652406
0.5407461919	0.1872972335
0.5614744579	0.1862858914
0.582888785	0.1847992092
0.6038385262	0.1828986914
0.6241084781	0.1806254835
0.6466148037	0.1775792383
0.6668377383	0.1743491794
0.6884300375	0.1703536152
0.7079958698	0.1662122875
0.7293864925	0.1610736977
0.7495134015	0.1556056937
0.7705518206	0.1491695939
0.7911207208	0.1420890692
0.8126544531	0.1337416767
0.8333939967	0.124682101
0.8546031754	0.1142398805
0.8756367315	0.102543356
0.894964385	0.09046151302
0.9171160571	0.0748571717
0.9270224169	0.06722901236
0.9369287767	0.05918895658
0.9474910224	0.05016821268
0.9580532681	0.04070676825
0.968162685	0.03127845583
0.9782721019	0.02154611739
0.9891360509	0.01084087029
1	0


==> CircleDistanceGraphkappa-100.dat.tex <==
0	0
0.005449288542	0.005422753685
0.01089857708	0.01069412936
0.01634786562	0.0156967261
0.02179715417	0.02036259996
0.03127994781	0.02762775197
0.04076274146	0.03388129423
0.05142713469	0.0399013737
0.06209152792	0.04506326145
0.07282661167	0.04957507987
0.08356169542	0.05353939581
0.104929819	0.06018819916
0.1247408048	0.06525132517
0.1452539331	0.0696740016
0.1664686398	0.07357354185
0.1876153106	0.07691984848
0.2093672608	0.0799035968
0.2285263904	0.08220844588
0.2500950325	0.08449272111
0.2717522375	0.0864974098
0.2926229675	0.08818693707
0.3115755898	0.08953534498
0.3341120908	0.09092863335
0.3532034633	0.09194367864
0.3754112681	0.09294667553
0.3950689383	0.09368384937
0.4166365181	0.09433774222
0.4371739544	0.09481548005
0.4586026146	0.09516779519
0.478280814	0.09536261383
0.4995064104	0.09543636253
0.5215538398	0.09536373386
0.5407461919	0.09517620191
0.5614744579	0.09484207269
0.582888785	0.09435036115
0.6038385262	0.09372081386
0.6241084781	0.0929663386
0.6466148037	0.09195264699
0.6668377383	0.09087427649
0.6884300375	0.08953496932
0.7079958698	0.08814002157
0.7293864925	0.0863986349
0.7495134015	0.08453142184
0.7705518206	0.08231248421
0.7911207208	0.07984115894
0.8126544531	0.07688010884
0.8333939967	0.07359689316
0.8546031754	0.06970237333
0.8756367315	0.06516280799
0.894964385	0.06021772948
0.9171160571	0.05330316455
0.9270224169	0.04963434688
0.9369287767	0.04550109907
0.9474910224	0.04046073863
0.9580532681	0.03459865901
0.968162685	0.02802193713
0.9782721019	0.020305548
0.9837040764	0.01565056272
0.9891360509	0.01066138144
0.9945680255	0.005405689645
1	0


==> CircleDistanceGraphkappa-2.dat.tex <==
0	0
0.02179715417	0.02174627472
0.04076274146	0.04043359479
0.06209152792	0.06095083424
0.08356169542	0.08085496916
0.104929819	0.09974294862
0.1247408048	0.1163244632
0.1452539331	0.1324816485
0.1664686398	0.1480697588
0.1876153106	0.1624606748
0.2093672608	0.1760771867
0.2285263904	0.1870926773
0.2500950325	0.1984262609
0.2717522375	0.2087038276
0.2926229675	0.2175979598
0.3115755898	0.2248438099
0.3341120908	0.2324638964
0.3532034633	0.238097927
0.3754112681	0.2437314919
0.3950689383	0.2479130415
0.4166365181	0.2516506322
0.4371739544	0.2543979345
0.4586026146	0.2564328192
0.478280814	0.257561233
0.4995064104	0.2579889835
0.5215538398	0.2575677269
0.5407461919	0.2564814652
0.5614744579	0.2545512663
0.582888785	0.2517230203
0.6038385262	0.2481236193
0.6241084781	0.2438425817
0.6466148037	0.23814801
0.6668377383	0.2321641297
0.6884300375	0.2248417734
0.7079958698	0.2173481822
0.7293864925	0.2081903463
0.7495134015	0.1986217757
0.7705518206	0.1875999501
0.7911207208	0.1757847569
0.8126544531	0.1622842882
0.8333939967	0.1481669351
0.8546031754	0.1325904844
0.8756367315	0.1160172928
0.894964385	0.09983395145
0.9171160571	0.0802400473
0.9369287767	0.0618769656
0.9580532681	0.04158838269
0.9782721019	0.0216775007
1	0


==> CircleDistanceGraphkappa0.6.dat.tex <==
0	0
0.02179715417	0.02179033305
0.04076274146	0.04071801479
0.06209152792	0.06193269273
0.08356169542	0.0831719033
0.104929819	0.104151186
0.1247408048	0.1234195228
0.1452539331	0.1431421635
0.1664686398	0.163243095
0.1876153106	0.1829204933
0.2093672608	0.2027163516
0.2285263904	0.2197141068
0.2500950325	0.2382753182
0.2717522375	0.2562007558
0.2926229675	0.2726899708
0.3115755898	0.2868948978
0.3341120908	0.3026916255
0.3532034633	0.3150148901
0.3754112681	0.3279596336
0.3950689383	0.338019139
0.4166365181	0.3473729598
0.4371739544	0.354487224
0.4586026146	0.3598974246
0.478280814	0.3629521475
0.4995064104	0.3641206462
0.5215538398	0.3629698432
0.5407461919	0.3600282947
0.5614744579	0.3548906052
0.582888785	0.3475577296
0.6038385262	0.3385367146
0.6241084781	0.3282216891
0.6466148037	0.3151271166
0.6668377383	0.3020520222
0.6884300375	0.2868907988
0.7079958698	0.2722132511
0.7293864925	0.2552778548
0.7495134015	0.238606079
0.7705518206	0.2205204206
0.7911207208	0.2022777681
0.8126544531	0.1826720016
0.8333939967	0.1633721398
0.8546031754	0.1432786227
0.8756367315	0.1230542176
0.894964385	0.1042545865
0.9171160571	0.08250365233
0.9369287767	0.062904706
0.9580532681	0.04189798315
0.9782721019	0.02172114186
1	0


==> CircleDistanceGraphkappa0.9.dat.tex <==
0	0
0.02179715417	0.0217954478
0.04076274146	0.04075153484
0.06209152792	0.0620516117
0.08356169542	0.08346331288
0.104929819	0.1047321645
0.1247408048	0.1244031515
0.1452539331	0.1447096956
0.1664686398	0.1656285496
0.1876153106	0.1863770551
0.2093672608	0.2075858009
0.2285263904	0.2261279299
0.2500950325	0.2468092545
0.2717522375	0.2673188571
0.2926229675	0.2867751864
0.3115755898	0.3041108003
0.3341120908	0.32419328
0.3532034633	0.3406208278
0.3754112681	0.3588312842
0.3950689383	0.3738785342
0.4166365181	0.3888193222
0.4371739544	0.4010007646
0.4586026146	0.4108890856
0.4684417143	0.4142514189
0.478280814	0.4167716604
0.4888936122	0.4184789364
0.4995064104	0.4190887204
0.5105301251	0.4185405388
0.5215538398	0.4168064592
0.5311500158	0.4143731961
0.5407461919	0.4111362774
0.5614744579	0.40171743
0.582888785	0.389125731
0.6038385262	0.3746787701
0.6241084781	0.3592121928
0.6466148037	0.3407741157
0.6668377383	0.3233606501
0.6884300375	0.3041057081
0.7079958698	0.2862033829
0.7293864925	0.2662479156
0.7495134015	0.2471825359
0.7705518206	0.2270162657
0.7911207208	0.2071117164
0.8126544531	0.1861131174
0.8333939967	0.1657636835
0.8546031754	0.144850894
0.8756367315	0.1240287879
0.894964385	0.1048373461
0.9171160571	0.08278797371
0.9369287767	0.06302936951
0.9580532681	0.04193451589
0.9782721019	0.02172620799
1	0


==> CircleDistanceGraphkappa0.dat.tex <==
0	0
0.02179715417	0.02178012293
0.04076274146	0.04065141907
0.06209152792	0.06169850377
0.08356169542	0.0826052204
0.104929819	0.1030397168
0.1247408048	0.1215724143
0.1452539331	0.1402649814
0.1664686398	0.158983416
0.1876153106	0.1769393633
0.2093672608	0.1945940273
0.2285263904	0.2093944819
0.2500950325	0.2251462671
0.2717522375	0.2399229211
0.2926229675	0.25311323
0.3115755898	0.2641503075
0.3341120908	0.2760530011
0.3532034633	0.28505614
0.3754112681	0.2942371288
0.3950689383	0.3011706462
0.4166365181	0.3074559354
0.4371739544	0.3121298789
0.4586026146	0.3156217363
0.478280814	0.3175691928
0.4995064104	0.3183095035
0.5215538398	0.3175804232
0.5407461919	0.3157055274
0.5614744579	0.3123921036
0.582888785	0.3075784975
0.6038385262	0.3015225388
0.6241084781	0.2944200056
0.6466148037	0.2851369647
0.6668377383	0.2755788721
0.6884300375	0.2641471675
0.7079958698	0.2527375043
0.7293864925	0.2391730452
0.7495134015	0.225422893
0.7705518206	0.2100878617
0.7911207208	0.1942076239
0.8126544531	0.1767150537
0.8333939967	0.1591024042
0.8546031754	0.1403932376
0.8756367315	0.1212234133
0.894964385	0.1031398107
0.9171160571	0.08195050102
0.9369287767	0.06265932534
0.9580532681	0.04182543048
0.9782721019	0.02171102869
1	0


==> CircleMagGraphK0.table.tex <==
0.03441655922	1.006992903
0.06883311845	1.014023161
0.1032496777	1.021090855
0.1376662369	1.028196064
0.2064993554	1.042519344
0.2753324738	1.05699362
0.4129987106	1.086397557
0.5506649475	1.116412503
0.825997421	1.178292547
1.101329895	1.242665142
1.580460521	1.360704823
2.059591147	1.486474266
3.137256148	1.797802728
4.222064611	2.150552149
5.301717169	2.539196305
6.302693295	2.930576365
7.339146095	3.364112192
8.411047064	3.838781722
9.479510432	4.334210465
10.57855634	4.86247794
11.54659657	5.339994851
12.63638059	5.887798399
13.73063937	6.445628608
14.78516046	6.988083794
15.74276664	7.483234833
16.88145301	8.07365074
17.84606973	8.574271563
18.96814829	9.156352128
20	9.690899262

